How To Optimize My Blockchain? A Multi-Level Recommendation Approach

Aside from the conception of new blockchain architectures, existing blockchain optimizations in the literature primarily focus on system or data-oriented optimizations within prevailing blockchains. However, since blockchains handle multiple aspects ranging from organizational governance to smart contract design, a holistic approach that encompasses all the different layers of a given blockchain system is required to ensure that all optimization opportunities are taken into consideration. In this vein, we define a multi-level optimization recommendation approach that identifies optimization opportunities within a blockchain at the system, data, and user level. Multiple metrics and attributes are derived from a blockchain log and nine optimization recommendations are formalized. We implement an automated optimization recommendation tool, BlockOptR, based on these concepts. The system is extensively evaluated with a wide range of workloads covering multiple real-world scenarios. After implementing the recommended optimizations, we observe an average of 20% improvement in the success rate of transactions and an average of 40% improvement in latency.

==> content/AllExperiments.tex <==

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\renewcommand{\arraystretch}{0.3}
\renewcommand{\arraystretch}{1.2}
% Table generated by Excel2LaTeX from sheet 'Sheet4 (2)'
%\begin{table}[htbp]
\begin{table*}[ht]
  \centering
  \caption{Experiments with the synthetic workload}
  \small\addtolength{\tabcolsep}{-5pt}
  \scalebox{0.7}{%
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|M{8em}|}{\textbf{Experiment Number}} & \multicolumn{1}{M{15em}|}{\textbf{Control variable}} & \multicolumn{1}{M{15em}|}{\textbf{Value}} & \multicolumn{1}{M{15em}|}{\textbf{Optimizations recommended}} \\
    \hhline{|=|=|=|=|}
    \multirow{1} & \multicolumn{1}{c|}{\multirow{Endorsement}} & \multicolumn{1}{c|}{\multirow{P1}}    & Endorser restructure \\
         & Policy      &           & Activity reordering \\
        %      \multirow{1} & \multicolumn{1}{c|}{\multirow{Endorsement}} & \multicolumn{1}{c|}{\multirow{AND(Org1, OR(Org2,  }}    & Endorsement policy optimization \\
        %  & Policy      &  Org3,Org4))         & Activity reordering \\
%          &  No: of orgs     &  4         & All optimizations \\
%          &       &       & 27    & All optimizations \\
    \hline
    \multirow{2} & \multicolumn{1}{c|}{\multirow{Endorsement Policy / }} & \multicolumn{1}{c|}{\multirow{P2 / 6 }}    & Endorser restructure \\
          & Endorser dist skew      &          & Activity reordering \\
   %       &   Endorser dist skew     &     6       & All optimizations \\
%          &       &       & 31    & All optimizations \\
    \hline
    \multirow{3} & \multicolumn{1}{c|}{\multirow{Endorsement }} & \multicolumn{1}{c|}{\multirow{P3}}    & Transaction rate control \\
          & Policy      &             & Activity reordering \\
  %        &  No: of orgs     & 4     & All optimizations \\
%          &       &       & 35    & All optimizations \\
    \hline
    \multirow{4} & \multicolumn{1}{c|}{\multirow{No: of orgs}} & \multirow{2}     & Activity reordering \\
%          & Organizations       &       &     &  \\
%          &       &       & 38    & All optimizations \\
    \hline
    \multirow{5} & \multicolumn{1}{c|}{\multirow{No: of orgs }} & \multirow{4}     & Transaction rate control \\
%          & Organizations       &       &     &  \\
%          &       &       & 41    & All optimizations \\
    \hline
%     \multirow{5} & \multicolumn{1}{c|}{\multirow{Endorser }} & \multirow{0} & 37    & Block size adaptation \\
%           & distribution      &       & 38    & Activity reordering \\
%           &       &       & 39    & All optimizations \\
%     \hline
%     \multirow{6} & \multicolumn{1}{c|}{\multirow{Endorser }} & \multirow{2} & 40    & Block size adaptation \\
%           & distribution      &       & 41    & Activity reordering \\
%           &       &       & 42    & Endorsement policy optimization \\
%           &       &       & 43    & All optimizations \\
%     \hline
    \multirow{6} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Uniform}}     & Activity reordering \\
%          &       &       & 43    & Activity reordering \\
%          &       &       & 44    & All optimizations \\
    \hline
    \multirow{7} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Read-heavy}}     & Activity reordering \\
%          &       & -Heavy      &     &  \\
%          &       &       & 47    & All optimizations \\
    \hline
    \multirow{8} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Update-heavy}}     & Transaction rate control \\
%          &       &          & Delta-writes possibility \\
%          &       &       & 50    & All optimizations \\
    \hline
    \multirow{9} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Insert-heavy}}     & Activity reordering \\
%          &       & -Heavy      &     &  \\
%          &       &       & 53    & All optimizations \\
    \hline
    \multirow{10} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{RangeRead-heavy}}    & Activity reordering \\
%          &       & -Heavy      &     &   \\
%          &       &       & 56    & All optimizations \\
    \hline
    \multirow{11} & \multicolumn{1}{c|}{\multirow{Key distribution}} & \multirow{0}     & Activity reordering \\
%          & Distribution      &       &     &   \\
%          &       &       & 59    & All optimizations \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{ }} & \multirow{}     & Transaction rate control \\
  12        & Key      &           & Activity reordering \\
 %         & Distribution       & 2          & Delta-writes possibility \\
          &  distribution     &  2        & Smart contract partition \\
 %         &       &          & All optimizations \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Block size adaptation \\
  13        & Block size      &  50        & Activity reordering \\
%%          &       &           & All optimizations \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Block size adaptation \\
  14        & Block size      &  100         & Activity reordering \\
  %        &       &           & All optimizations \\
    \hline
     \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
 15         & Block size       &   300        & Activity reordering \\
   %       &       &          & All optimizations \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
   16       & Block size      & 500          & Activity reordering \\
  %        &       &          & Delta-writes possibility \\
  %        &       &           & All optimizations \\
    \hline
     \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
  17        &  Block size     &  1000        & Activity reordering \\
 %         &       &          & All optimizations \\
    \hline
    18    & \multicolumn{1}{c|}{Send rate} & 50       & Activity reordering \\
    \hline
    \multirow{19} & \multicolumn{1}{c|}{\multirow{Send rate}} & \multirow{100}     & Activity reordering \\
  %        &       &           & Delta-writes possibility \\
    \hline
     20    & \multicolumn{1}{c|}{Send rate} & 300       & Activity reordering \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
   21       &  Send rate     & 500          & Activity reordering \\
   %       &       &         & All optimizations \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Block size adaptation \\
              &       &          & Transaction rate control \\
   22       &  Send rate     &  1000        & Activity reordering \\
    %      &       &          & Delta-writes possibility \\
  %        &       &           & All optimizations \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multicolumn{1}{c|}{\multirow{}}     & Block size adaptation \\
           23       &  Send rate     &  500, 1000       & Transaction rate control \\
          &       &          & Activity reordering \\
   %       &       &         & All optimizations \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multicolumn{1}{c|}{\multirow{}}    & Transaction rate control \\
           24       &  Transaction     &  70\%        & Activity reordering \\
          & distribution      &           & Client resource boost \\
   %       & skew      &         & All optimizations \\
    \hline
    \end{tabular}}%
  \label{snyexperiments}%
\end{table*}%

\newline
\newline
\newline

\begin{figure*}[ht]
\minipage{0.3\linewidth}
\includegraphics[width=\linewidth]{figures/endpol.pdf}
\captionsetup{justification=centering} 
\captionsetup{labelfont={bf}}
\caption{Performance without and with endorsement policy optimization}
%\caption{Effect of the \mbox{number} of organizations}
\label{endpol}
\endminipage\hfill
\minipage{0.3\linewidth}
\includegraphics[width=\linewidth]  {figures/clientdist.pdf}
\captionsetup{justification=centering} 
\captionsetup{labelfont={bf}}
\caption{Performance without and with client resource boost}
\label{clientdist}
\endminipage\hfill
\minipage{0.3\linewidth}
\includegraphics[width=\linewidth]  {figures/blksz.pdf}
\captionsetup{justification=centering} 
\captionsetup{labelfont={bf}}
\caption{Performance without and with block size optimization}
\label{blksz}
\endminipage\hfill
\end{figure*}

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/blksz.pdf}
% \caption{Performance without and with block size optimization}
% \label{blksz}
% \end{figure*}


\begin{figure*}[ht]
\centering
\includegraphics[width=0.9\linewidth]{figures/ratecntrl.pdf}
\caption{Performance without and with transaction rate control  optimization}
\label{ratecntrl}
\end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=0.9\linewidth]{figures/rord.pdf}
\caption{Performance without and with transaction reordering optimization}
\label{rord}
\end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=0.8\linewidth]{figures/allopt.pdf}
\caption{Performance without and with all recommended optimizations}
\label{allopt}
\end{figure*}

==> content/coverletter.tex <==

\onecolumn
\noindent
{\large We would like to thank all the reviewers for their insightful feedback which helped us to improve our paper. All the revisions requested in the meta review are addressed. Additionally, we also included some of the suggestions in the main review. In the paper, all major changes are marked with \textcolor{blue}{blue} text. Line numbers are added in the paper for ease of reference.
\noindent
All the changes made to the paper are listed here. We show the reviewer's remarks in \textbf{bold} text and our revision in \textcolor{blue}{blue} text.}

\noindent
\textbf{Meta review:}

\noindent
\textbf{R1O2/R1O3: Clarify variables and thresholds.}

\noindent
{\large\textcolor{blue}{In Section 6 (Lines 745 - 748), the values of the thresholds for all our experiments are added. We included a new Table 4 that shows the settings including the control variable values used to implement each of the recommended optimizations for all our experiments. This gives the reader a better understanding of our experiments. A \textit{Future Work} discussion is also added in Section 9 (line numbers 1119 - 1123) to include the reviewer's suggestions regarding automated thresholds settings.}

\noindent
\textbf{R1O4: Make figures more readable.}

\noindent
{\large\textcolor{blue}{We increased the size of Figures 10-12 and 16-19 and increased the font size of Figures 7-9, 13-15 and 18 to improve readability.}}

\noindent
\textbf{R1 Minor remarks: I suggest replacing adaption with adaptation throughout the paper.}

\noindent
{\large\textcolor{blue}{We have replaced adaption with adaptation throughout the paper.}}


\noindent
\textbf{R2O1: Clarify the novelty claim.}

\noindent
{\large\textcolor{blue}{In the third paragraph of the introduction, we rephrased our initial claim to clarify the misunderstanding that the process level is not ignored in the literature but rather a comprehensive approach is lacking. The statement \textit{"Further, beyond mere system-level tuning and data remodeling, another dimension of blockchain optimizations exists that has, however, been ignored so far."} is changed to \textit{"Further, the literature falls short for an end-to-end optimization approach that includes not only system-level tuning and data remodeling but also process model redesign."} (See lines 22 - 24 in Section 1).}}

\noindent
\textbf{R2O2: Clarify application modelling.}

\noindent
{\large\textcolor{blue}{In Section 4.2, lines 347 - 354, we clarify the process of CaseID generation. We included sources from process mining documentations, case studies and research papers [4,8,17,19,44] which discuss the process of identifying the common element to use as caseID based on the domain knowledge. Due to our interest in a transactional perspective of the process model, the common element is chosen from the function arguments and read-write sets. We also give an example of the SCM scenario to explain how a suitable choice of the common element is made based on domain knowledge.} }

\noindent
\textbf{R2O4: Clarify end-to-end process.}

\noindent
{\large\textcolor{blue}{We modified Section 4.5 and added Figure 6 to explain where the recommended optimizations can be applied on a live Fabric Network without restarting. An automated workflow engine, client transaction monitoring, smart contract upgrades and Fabric \textit{update transactions} can be used to implement all the optimizations on the fly. We also explicitly state in lines 616 - 619 that we restart the Fabric network in our experiments since our evaluation runs in an experimental environment. Also, the limitations in Section 7 (lines 1046 - 1052) are expanded to discuss the scenario of workload fluctuations and optimization implementation delays. Furthermore, a \textit{Future Work} discussion is added in Section 9 (lines 1126 -1128) to include the reviewer's suggestions.}}

\noindent
\textbf{R2O5: Clarify relevance of the LAP workload.}

\noindent
{\large\textcolor{blue}{We expanded Section 5.1.3 (lines 728 - 733) and explain the security and decentralization requirements of an automated loan application system that makes it a suitable use-case for blockchains. Relevant references [33, 58, 82, 83] are also added for the stated examples.}}

\noindent
\textbf{R3O1: Rework the abstract and introduction to clarify the problem being solved.}

\noindent
\textcolor{blue}{We extensively modified the abstract and introduction to clarify the problem statement. In both the abstract and the introduction, we now use terms such as "existing blockchains", "of a given blockchain", "within a blockchain" etc. to emphasize that our optimization recommendations are focused on a particular blockchain rather than optimizing across different blockchains. Further, in the introduction, redundancy is removed.}}

\noindent
\textbf{R3O2/R3O3/R3O4: Comment on the limitations of a logging-based approach and clarify log timestamps.}

\noindent
{\large\textcolor{blue}{We modified Sections 4.1 (line 312), 4.2 (lines 360 - 364) and 4.3 (line 378) to clarify the log timestamps. The client timestamps available in the log are used for deriving the transaction rate (Section 4.3 line 378) and the commit order is used to derive the process model. The limitations in Section 7 (lines 1034 - 1040) are expanded to discuss the scenario where an application is not based on a process model and log analysis may not be beneficial for some optimizations. We also added a \textit{Future Work} discussion in Section 9 (line 1123 - 1125) to include the reviewer's suggestions regarding additional logging.}}

\noindent
\textbf{R3O5: Comment on the generality of the transaction-centric approach.}

\noindent
{\large\textcolor{blue}{We expanded Section 4 (lines 281 - 291) to discuss the generality of a transaction-centric approach. Since blockchains are defined as a distributed record of transactions and smart contract executions result in transactions, a transactional perspective is appropriate for log analysis in blockchains.}}




==> content/tableold.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\renewcommand{\arraystretch}{0.3}
\renewcommand{\arraystretch}{1.2}
% Table generated by Excel2LaTeX from sheet 'Sheet4 (2)'
%\begin{table}[htbp]
\begin{table}[t]
  \centering
  \caption{Experiments with the synthetic workload}
  \small\addtolength{\tabcolsep}{-5pt}
  \scalebox{0.7}{%
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|M{5.5em}|}{\textbf{Experiment Number}} & \multicolumn{1}{M{10em}|}{\textbf{Control variable}} & \multicolumn{1}{M{10em}|}{\textbf{Value}} & \textbf{Optimizations recommended} \\
    \hhline{|=|=|=|=|}
    \multirow{1} & \multicolumn{1}{c|}{\multirow{Endorsement}} & \multicolumn{1}{c|}{{P1}}    & Endorser restructuring \\
         & Policy      &           & Activity reordering \\
    \hline
    \multirow{2} & \multicolumn{1}{c|}{\multirow{Endorsement Policy / }} & \multicolumn{1}{c|}{\multirow{P2 / 6 }}    & Endorser restructuring \\
          & Endorser dist skew      &          & Activity reordering \\
    \hline
   % \multirow{3} & \multicolumn{1}{c|}{\multirow{Endorsement }} & \multicolumn{1}{c|}{\multirow{P3}}    & Transaction rate control \\
    %      & Policy      &             & Activity reordering \\
  %  \hline
   % \multirow{4} & \multicolumn{1}{c|}{\multirow{No: of orgs}} & \multirow{2}     & Activity reordering \\
  %  \hline
%5,6,7,8,9
    \multirow{3} & \multicolumn{1}{c|}{\multirow{No: of orgs }} & \multirow{4}     & Transaction rate control \\
    \hline
   % \multirow{6} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Uniform}}     & Activity reordering \\
    %\hline
    \multirow{4} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Read-heavy}}     & Activity reordering \\
    \hline
    \multirow{5} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Update-heavy}}     & Transaction rate control \\
    \hline
    \multirow{6} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{Insert-heavy}}     & Activity reordering \\
    \hline
    \multirow{7} & \multicolumn{1}{c|}{\multirow{Workload}} & \multicolumn{1}{c|}{\multirow{RangeRead-heavy}}    & Activity reordering \\
    \hline
  %  \multirow{11} & \multicolumn{1}{c|}{\multirow{Key distribution}} & \multirow{0}     & Activity reordering \\
  %  \hline
  %12,13
    \multirow{} & \multicolumn{1}{c|}{\multirow{ }} & \multirow{}     & Transaction rate control \\
  8        & Key      &           & Activity reordering \\
          &  distribution skew    &  2        & Smart contract partitioning \\
    \hline
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Block size adaptation \\
  9        & Block count      &  50        & Activity reordering \\
    \hline
%    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Block size adaptation \\
%  14        & Block size      &  100         & Activity reordering \\
%    \hline
%15
     \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
 10         & Block count       &   300        & Activity reordering \\
    \hline
%    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
%   16       & Block size      & 500          & Activity reordering \\
%    \hline
%17, 18
     \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
  11        &  Block count     &  1000        & Activity reordering \\
    \hline
    12    & \multicolumn{1}{c|}{Send rate} & 50       & Activity reordering \\
    \hline
    %\multirow{19} & \multicolumn{1}{c|}{\multirow{Send rate}} & \multirow{100}     & Activity reordering \\
    %\hline
    %20
     13    & \multicolumn{1}{c|}{Send rate} & 300       & Activity reordering \\
    \hline
%    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Transaction rate control \\
%   21       &  Send rate     & 500          & Activity reordering \\
%    \hline
%22
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multirow{}     & Block size adaptation \\
              &       &          & Transaction rate control \\
   14       &  Send rate     &  1000        & Activity reordering \\
    \hline
%    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multicolumn{1}{c|}{\multirow{}}     & Block size adaptation \\
%           23       &  Send rate     &  500, 1000       & Transaction rate control \\
%          &       &          & Activity reordering \\
%    \hline
%24
    \multirow{} & \multicolumn{1}{c|}{\multirow{}} & \multicolumn{1}{c|}{\multirow{}}    & Transaction rate control \\
           15       &  Transaction     &  70\%        & Activity reordering \\
          & distribution skew    &           & Client resource boost \\
    \hline
    \end{tabular}}
  \label{snyexperiments}
\end{table}%

